Construct Dynamic Graphs for Hand Gesture Recognition via Spatial-Temporal Attention

We propose a Dynamic Graph-Based Spatial-Temporal Attention (DG-STA) method for hand gesture recognition. The key idea is to first construct a fully-connected graph from a hand skeleton, where the node features and edges are then automatically learned via a self-attention mechanism that performs in both spatial and temporal domains. We further propose to leverage the spatial-temporal cues of joint positions to guarantee robust recognition in challenging conditions. In addition, a novel spatial-temporal mask is applied to significantly cut down the computational cost by 99%. We carry out extensive experiments on benchmarks (DHG-14/28 and SHREC'17) and prove the superior performance of our method compared with the state-of-the-art methods. The source code can be found at https://github.com/yuxiaochen1103/DG-STA.

==> network_structure.tex <==
\section{Network Structure and Implementation Details}
\label{sec:arch}

Our network structure is shown in Figure \ref{fig:arch}. We set the head numbers of both spatial and temporal attention model as 8, and the dimension $d$ of query, key, and value as 32. The Layer Normalization~\cite{ln} is used to normalize network intermediate outputs. The input 3D coordinates of all hand joints are projected to 128D initial node features. Then the obtained initial node features are added with the S-PE and fed to spatial attention model, resulting new 256D node features. The output of spatial attention model are projected to 128D vectors and then added with the T-PE. The temporal attention model takes the results as input, and updates node features again. Finally, we average-pool the features of all nodes as a vector and feed it to a FC layer for classification.

\begin{figure}
\includegraphics[width=1\textwidth]{images/network.pdf}
\caption{The architecture of our network. S-PE and T-PE represent spatial position embedding and temporal position embedding, respectively. For details, please refer to Section \ref{sec:arch}.}
\label{fig:arch}
\end{figure}
